Application of Quantum Process Calculus to Higher Dimensional Quantum Protocols

We describe the use of quantum process calculus to describe and analyze quantum communication protocols, following the successful field of formal methods from classical computer science. We have extended the quantum process calculus to describe d-dimensional quantum systems, which has not been done before. We summarise the necessary theory in the generalisation of quantum gates and Bell states and use the theory to apply the quantum process calculus CQP to quantum protocols, namely qudit teleportation and superdense coding.

==> eptcsdata.tex <==
\providecommand{\firstpage}{15}
\providecommand{\publicationstatus}{R. Duncan and P. Panangaden (Eds.)\\
Quantum Physics and Logic 2012 (QPL2012)\\
EPTCS 158, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.158.2}{10.4204/EPTCS.158.2}}
\pdfoutput=1

